Blockchain-based Secure Client Selection in Federated Learning

Despite the great potential of Federated Learning (FL) in large-scale distributed learning, the current system is still subject to several privacy issues due to the fact that local models trained by clients are exposed to the central server. Consequently, secure aggregation protocols for FL have been developed to conceal the local models from the server. However, we show that, by manipulating the client selection process, the server can circumvent the secure aggregation to learn the local models of a victim client, indicating that secure aggregation alone is inadequate for privacy protection. To tackle this issue, we leverage blockchain technology to propose a verifiable client selection protocol. Owing to the immutability and transparency of blockchain, our proposed protocol enforces a random selection of clients, making the server unable to control the selection process at its discretion. We present security proofs showing that our protocol is secure against this attack. Additionally, we conduct several experiments on an Ethereum-like blockchain to demonstrate the feasibility and practicality of our solution.

==> communication.tex <==
\medskip
\noindent\textbf{Performance.} We now analyze the communication, time complexities, and the costs associated with the use of blockchain.

% , and the blockchain in our protocol.
\noindent\emph{Communication complexity.} \underline{Client-server}. There is a one-time cost of $O(\log n)$, associated with the Merkle proof for the registration from the server.
In each training round, each client will communicate with the server   a VRF proof \tn{output + pk?} ($O(1)$), a Merkle proof in the initial selection (size $O(\log m_1)$, where $m_1 = |\calP_t| < m$), possibly a $O(\log m_2)$ Merkle proof, where $m_2 < m$ is the number of dispute clients. Thus, the communication cost for each round is $O(\log m)$ per client, where  $m = |\calP_f|$, the number of selected clients.  Similarly, the communication cost for the server is a one-time cost $O(n \log n)$ for registration and $O(n \log m)$ for each round. 
%
\underline{Communication with blockchain nodes.} The server will need to retrieve a full copy of the blockchain, incuring an $O(\kappa b)$  cost to download $O(\kappa)$ blocks in each round, where $b$ is the average size of each block. \tn{the server does not need the whole block right?
} Clients can use Simple Payment Verification (SPV) \cite{nakamoto2008bitcoin}, a lightweight verification protocol, and only need to download headers of the blocks. Hence, each client incurs only a communication cost $O(\kappa)$ per training round.
%In each training round, they download $\tau$ blocks. 
%
%Let $b$ be the size of a block. The communication complexity to maintain the blockchain is $O(\kappa b)$ (as each training round last $\tau = O(\kappa)$ blocks). 
% Since the size of the block is large (e.g., the maximum size of a Bitcoin block is $2$MB), it is not feasible for the clients to maintain the full blockchain. Fortunately, \cite{nakamoto2008bitcoin} introduces the Simple Payment Verification (SPV) technique to allow a lightweight client to verify that a transaction is included in the Bitcoin blockchain by only maintaining the block headers with constant size (e.g., the Bitcoin block header is $80$ bytes). The communication complexity to maintain the block headers in each training round is $O(\kappa)$ 
%In each round, the server sends and receives a message of size $O(\log n)$  to each selected client. Thus, the comumication is $O(\log n)$ for each client and $O(n \log n)$ for the server.
%, where $m = cn$ is the number of selected clients.
Combining all communication cost, the communication complexity of the server and each client are $O(n \log m + \kappa b)$ (since $m_1,m_2 \le m$) and client is $O(\log m + \kappa)$, respectively.


\noindent\emph{Time complexity.} 
In a training round, each client takes $O(\kappa)$ to compute the randomness,  $O(1)$ to compute the VRF, and $O(\log m)$ to verify the Merkle proofs. Similarly, the server takes $O(\kappa)$ to compute the randomness,  $O(m)$ \tn{$m_1$?} to verify the VRF proofs of the selected clients, and constructs Merkle tree proofs for all clients in $O(n \log m)$. 
Thus, the time complexity of the server and each client per training round are $O(\kappa +m + n \log m)$ and $O(\kappa + \log m)$, respectively. 


%In the randomness extraction step, the server and the clients need to compute the randomness in $O(\kappa)$ time complexity.
%In the random election step, each client needs to compute the VRF in $O(1)$\footnote{The time complexity of the VRF depends on the size of the input, i.e., the randomness, which we consider as a constant.} time complexity. In the initial commitment step and the final commitment step, the server needs to construct two Merkle trees in $O(m_1)$, $O(m_2)$ time complexity, respectively. Each client needs to verify the Merkle paths in $O(\log m_1)$, $O(\log m_2)$  time complexity,  respectively. In total, 
%%besides the cost to maintain the blockchain, 
%the time complexity of the server is $O(\kappa +m)$ (since $m_1,m_2 \le m$), the time complexity of each client is $O(\kappa + \log m)$. 


%\noindent\emph{The storage complexity to maintain the blockchain.} In our protocol, both the server and the clients need to maintain a blockchain. This require a huge amount of storage. For example, the blockchain size of Ethereum is 1123.28 GB\footnote{\url{https://ycharts.com/indicators/ethereum_chain_full_sync_data_size}, December 18, 2021}. Thus, it is not feasible for the clients to maintain the full blockchain.
%
%\noindent\underline{SPV clients.} Fortunately, the previous work introduces the Simple Payment Verification (SPV) technique to allow a lightweight client to verify that a transaction is included in the Bitcoin blockchain, without downloading the entire blockchain. More concretely, the SPV client only downloads and stores the block headers in which, each block header consists of a pointer to the previous block, the PoW puzzle, and a small commitment on the list of transactions. The SPV clients can verify if a transaction is included on the blockchain based on a proof that is provided by a full node, i.e., the node that downloads all the entire blockchain.
%
%To enable the SPV clients, we modify our protocol in Fig.\ref{alg:protocol} as follows: 1) extract the randomness based on the block headers instead of the full blocks; 2) the server needs to provide the proofs that the initial commitment transaction and the final commitment transaction is included on the blockchain. 

%By using the SPV clients, we can reduce the cost to maintain the blockchain for the clients. 

\noindent\emph{Blockchain's storage and computation (gas) costs.}
In our protocol, the size of an initial selection transaction, a dispute transaction, and a final selection transaction are $O(1)$, $O(\log 1)$, and $O(1)$, respectively.
% The size of a dispute transaction is  $O(\log n)$.
The time to verify an initial selection transaction, a dispute transaction, and a final selection transaction is $O(1)$, $O(\log n)$, and $O(m_2)$ (where $m_2$ is the number of dispute clients), respectively.


%There are three types of transactions in our protocol:
%\begin{itemize}
%%	\item \emph{Registration transaction (with size $O(1)$)}. To verify this transaction, the miners check if it is submitted by the server. Thus, the time complexity to verify this transaction is $O(1)$.  
%	\item \emph{Initial commitment transaction} (with size $O(1)$).  To verify this transaction, the miners check if it is submitted by the server. Thus, the time complexity to verify this transaction is $O(1)$. 
%	\item \emph{Dispute transaction} (with size $O(\log n)$). To verify this transaction, the miners check if 1) the Merkle tree path for the registration is correct, and 2) the VRF proof is correct. Thus, the time complexity to verify this transaction is $O(\log n)$. 
%	\item \emph{Final commitment transaction} (with size $O(1)$). To verify this transaction, the miners construct a Merkle tree from the public keys of the dispute clients. Thus, the time complexity to verify this transaction is $O(m_2)$, where $m_2$ is the number of dispute clients. 
%\end{itemize}

In each training round, the server submits one initial selection transaction and one final selection transactions. The clients submit $m_2$ dispute transaction. 
Thus, the storage and computational costs on blockchain of the server are $O(1)$ and $O(m_2)$, respectively. Thus,
the  total blockchain's cost for the clients is $O(m_2 \log n)$.

%We now analyze the storage and computation complexity on blockchain for honest nodes. 
%We consider two following cases of the server.
%\begin{itemize}
%	\item \emph{Honest server.} In this case, the honest clients does not submit any dispute transaction. The honest s
%	\item \emph{Malicious server.} In this case, the total number of transactions from honest parties is $O(m)$ (where $m$ is the number of disputed clients).
%\end{itemize}


%There are two types of nodes in the blockchain system, called \emph{full nodes} and \emph{SPV nodes}. 
%Each full node downloads, verifies, and stores all information on the blockchain. On the other hand, each SPV node stores a header chain that only consists of the block headers. 
%Each block header contains the information of a pointer to the previous blocks, the PoW puzzle, and a small commitment on the list of transactions. By using the commitment, the SPV can verify if a transaction is included in the block. 
